Position: Cracking the Code of Cascading Disparity Towards Marginalized Communities

The rise of foundation models holds immense promise for advancing AI, but this progress may amplify existing risks and inequalities, leaving marginalized communities behind. In this position paper, we discuss that disparities towards marginalized communities - performance, representation, privacy, robustness, interpretability and safety - are not isolated concerns but rather interconnected elements of a cascading disparity phenomenon. We contrast foundation models with traditional models and highlight the potential for exacerbated disparity against marginalized communities. Moreover, we emphasize the unique threat of cascading impacts in foundation models, where interconnected disparities can trigger long-lasting negative consequences, specifically to the people on the margin. We define marginalized communities within the machine learning context and explore the multifaceted nature of disparities. We analyze the sources of these disparities, tracing them from data creation, training and deployment procedures to highlight the complex technical and socio-technical landscape. To mitigate the pressing crisis, we conclude with a set of calls to action to mitigate disparity at its source.

==> sections/Issues.tex <==


\begin{enumerate}
    \item Jailbreak
    \item Unsafe content
    \item 
\end{enumerate}

==> sections/Section_2_Related_Work.tex <==
\todo[inline]{Do we need related work for a position paper?}

\noindent \textbf{Bias and Fairness in Machine Learning}


\noindent \textbf{Responsible Development of Foundation Models}



==> sections/Section_3_Foundation_vs_Traditional.tex <==
%\textit{Foundation models} are large AI models trained on enormous quantities of unlabeled data—usually through self-supervised learning. This process results in generalized models capable of a wide variety of tasks, such as image classification, natural language processing, and question-answering, with remarkable accuracy. On the other hand, \textit{traditional ML models}, typically focus on solving specific tasks using supervised or unsupervised learning methods, and they are trained on curated datasets relevant to the task.


While both traditional ML models and foundation models can exhibit disparities, the nature and sources of these disparities can differ significantly. Foundation models, due to their scale and complexity, present unique challenges in terms of disparity identification, mitigation, and societal impact. In this section, we discuss the nature and sources of these disparities on marginalized community and how they can differ in several key ways. 

\begin{itemize}
    \item \textbf{Data Source}: 
    \item \textbf{Learning procedure}: 

    \item \textbf{Measurement}: The size and complexity of foundation models make it difficult to comprehensively assess their disparities. Traditional disparity detection methods often fall short due to the model's ability to mask disparities in subtle ways. Foundation models, specifically multi-modal versions, often process multiple types of data, such as text, images, and audio. This means that disparities can manifest in different forms, making it challenging to develop a universal evaluation framework. Additionally, disparities can emerge in different contexts and evolve over time. Static evaluation methods may not capture these dynamic patterns. Finally, currently, no widely accepted set of metrics exists to measure disparities in foundation models. Different researchers and organizations may prioritize different fairness criteria, which makes comparisons and bench marking very difficult and challenging.
    %\item \textbf{Resource Barriers (Data, infrastructure, and skills)} Traditional ML models and foundation models require different type of resources, ranging from data to compute and skills. Foundation models require massive and diverse datasets for training, which can be expensive and challenging to acquire and curate. In addition, training foundation models necessitates powerful computing infrastructure, including TPUs, GPUs and specialized hardware accelerators, which can be costly to access and maintain. And finally, development and training of foundation models require teams with higher levels of expertise in machine learning which are relatively scarce and in high demand, while training traditional ML models often cheaper as it requires smaller dataset, infrastructure and smaller teams with more general ML skills.
    
    
    \item \textbf{Impact}: The impact of disparity in traditional models is often limited to the specific task or domain for which the model is trained. In foundation models, however, because these models are often used for more general-purpose tasks and can impact various downstream applications, the potential societal impact of their disparities can be much broader and more significant.
        
    \item \textbf{Monopoly Effects}: Unlike traditional ML models, training foundation models necessitates vast amounts of data and specialized hardware, often inaccessible to most organizations and researchers. This creates a high barrier to entry for marginalized communities, and leads to a concentration of power among a few large tech companies with the resources to develop and control these models. This concentration can stifle competition and innovation, as smaller players are often unable to challenge the dominance of large players with their proprietary foundation models. Moreover, as more organizations rely on foundation models from a few providers to power their products and services, a widespread dependence on these models emerges which lead to propagation of disparities in various downstream tasks that are stemmed from a single model. This can also create a lock-in effect, which makes it difficult to transition to alternative models or providers, as entire ecosystems become built upon a limited set of foundation models. This concentration of power grants a few companies significant control over the development and direction of AI research and applications while the root of disparities are the same and create a systematic way that disparities impact society. Finally, the monopoly effect raises concerns about the potential for these companies to prioritize commercial interests over social good. 
    
    
    \item \textbf{Long-term Impact}
    
    

\end{itemize}


